Language Models can Exploit Cross-Task In-context Learning for Data-Scarce Novel Tasks

Large Language Models (LLMs) have transformed NLP with their remarkable In-context Learning (ICL) capabilities. Automated assistants based on LLMs are gaining popularity; however, adapting them to novel tasks is still challenging. While colossal models excel in zero-shot performance, their computational demands limit widespread use, and smaller language models struggle without context. This paper investigates whether LLMs can generalize from labeled examples of predefined tasks to novel tasks. Drawing inspiration from biological neurons and the mechanistic interpretation of the Transformer architecture, we explore the potential for information sharing across tasks. We design a cross-task prompting setup with three LLMs and show that LLMs achieve significant performance improvements despite no examples from the target task in the context. Cross-task prompting leads to a remarkable performance boost of 107% for LLaMA-2 7B, 18.6% for LLaMA-2 13B, and 3.2% for GPT 3.5 on average over zero-shot prompting, and performs comparable to standard in-context learning. The effectiveness of generating pseudo-labels for in-task examples is demonstrated, and our analyses reveal a strong correlation between the effect of cross-task examples and model activation similarities in source and target input tokens. This paper offers a first-of-its-kind exploration of LLMs' ability to solve novel tasks based on contextual signals from different task examples.

==> old_format/results.tex <==
\section{Results and Analysis}

\subsection{Dataset and experimental setup}

\begin{table*}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{cccccccccccc}
\hline
 \backslashbox{TAR}{SRC}& Zero-shot & ARC-Easy & AG-news & BoolQ & Com-QA & C-POS & C-NER & MNLI & QQP  & RACE  & SST2 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}Llama-2-7b}                                                                                \\ \hline
ARC-Challenge        & 4.6       & \textbf{43.6}     & 33.6    & 35.0  & \textbf{43.6}           & 33.8          & 34.2          & 34.2 & 36.4 & 42.8  & 33.2 \\
Financial-Phrasebank & 34.1      & 43.5     & 62.1    & 40.9  & 14.6           & 1.4           & 0.4           & 62.7 & 44.7 & 53.4  & \textbf{65.0} \\
MedMCQA              & 4.2       & 31.4     & 26.8    & 28.0  & \textbf{33.0}           & 26.2          & 24.0          & 23.0 & 26.0 & 31.6  & 23.2 \\
SciQ                 & 8.0       & 59.0     & 45.4    & 49.0  & \textbf{65.6}           & 34.4          & 29.7          & 44.8 & 25.4 & 64.4  & 39.0 \\
Social-i-QA          & 41.1      & 44.3     & 40.1    & 40.3  & 48.5           & 38.9          & 39.1          & 38.9 & 39.7 & \textbf{49.1}  & 39.3 \\ \hline
Average              & 18.4      & 44.3     & 41.6    & 38.6  & 40.71          & 26.9          & 25.5          & 40.7 & 34.4 & \textbf{48.3} & 39.9 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}Llama-2-13b}                                                                               \\ \hline
ARC-Challenge        & 52.0      & \textbf{59.2}     & 50.6    & 54.6  & 57.4           & 50.6          & 49.8          & 49.2 & 52.8 & 56.8  & 50.8 \\
Financial-Phrasebank & 65.4      & 66.6     & 78.6    & 65.8  & 61.7           & 2.2           & 13.17         & 79.0 & \textbf{82.4} & 66.5  & 72.8 \\
MedMCQA              & 9.2       & 37.2     & 34.2    & 36.6  & 38.8           & 31.6          & 32.6          & 30.2 & 30.6 & \textbf{39.0}  & 31.4 \\
SciQ                 & 55.8      & \textbf{83.4}     & 76.2    & 80.2  & \textbf{83.4}           & 76.4          & 78.6          & 77.2 & 71.2 & 82.8  & 72.6 \\
Social-i-QA          & 55.3      & 60.8     & 55.8    & 56.5  & 63.5           & 56.8          & 55.9          & 53.5 & 55.7 & \textbf{63.7}  & 53.1 \\ \hline
Average              & 47.5      & 61.4     & 59.1    & 58.7  & 60.9           & 43.5          & 46.0          & 57.8 & 58.5 & \textbf{61.7} & 56.1 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}GPT3.5}                                                                               \\ \hline
ARC-Challenge        & 74.6      & 77.2     & 74.4    & 77.8  & 76.2           & 70.2          & 70.8          & 75.2 & 74.0 & \textbf{78.2}  & 72.6 \\
Financial-Phrasebank & 57.5      & 79.8     & \textbf{83.6}    & 78.6  & 82.0           & 50.3          & 64.3          & 72.2 & 74.2 & 73.4  & 75.6 \\
MedMCQA              & 49.6      & 49.8     & 48.5    & \textbf{50.0}  & 48.0           & 47.4          & 45.0          & 46.0 & 49.0 & 47.6  & 48.0 \\
SciQ                 & 91.2      & 91.4     & 89.9    & 90.6  & 91           & 87.8          & 82.0          & 88.8 & 89.8 & \textbf{92.2}  & 89.0 \\
Social-i-QA          & 76.0      & 76.2     & 75.8    & 74.0  & 75.2           & 73.2          & 74.0          & 75.8 & 73.0 & \textbf{77.2}  & 74.8 \\ \hline
Average              & 69.8      & \textbf{74.9}     & 74.5    & 74.2  & 74.5           & 65.8          & 67.2          & 71.6 & 72.0 & 73.7 & 72.0 \\ \hline
\end{tabular}
}
\caption{Accuracy for cross-task setup, $C$ is created using one source example. Source tasks are mentioned in columns and Target tasks are in rows. Cross-task prompting brings improvement over zero-shot prompting for certain source-target pairs. (Commonsense-QA, Conll2003-POS, Conll2003-NER abbreviated to Com-QA, C-POS and C-NER).}
\label{tab:cross-task}
\end{table*}
%\todo{Captions for Tables 1 and 2 do not clearly communicate what is show. Please elaborate properly.}
Our corpus of tasks consists of ten source and five target tasks. We considered ARC-Easy \cite{Clark2018ThinkYH}, AG-news \cite{Zhang2015CharacterlevelCN}, BoolQ \cite{clark-etal-2019-boolq}, Commonsense-QA \cite{talmor-etal-2019-commonsenseqa}, Conll2003-POS \cite{tjong-kim-sang-de-meulder-2003-introduction}, Conll2003-NER \cite{tjong-kim-sang-de-meulder-2003-introduction}, MNLI \cite{N18-1101}, QQP \cite{DBLP:journals/corr/abs-1907-01041}, RACE \cite{lai-etal-2017-race} and SST2 \cite{socher-etal-2013-recursive} to be our source tasks. Our target tasks are ARC-Challenge \cite{Clark2018ThinkYH}, Social-i-QA \cite{DBLP:journals/corr/abs-1904-09728}, SciQ \cite{SciQA2023}, MedMCQA \cite{pmlr-v174-pal22a} and Financial-Phrasebank \cite{Malo2014GoodDO}. In total this gives us 90 unique cross-task setups (See Appendix \ref{sec:appendix-dataset} for dataset details). Dataset size is standardised by sampling 10000 and 500 examples for each source and target task i.e. $|D_t|=10000$ and $|D_s|=500$. For our experiments, we used the 7-billion and 13-billion variants of Llama-2 \cite{touvron2023llama} for their easy access to the general public. We also utilise text-davinci-003 \cite{DBLP:journals/corr/abs-2005-14165} referred to as GPT3.5 in tables. We set the number of examples used to create $C$ as one for all our experiments (unless mentioned explicitly). 



\subsection{Does cross-task prompting work?}
\label{sec:cross-task-main-result}

As evident from Table \ref{tab:cross-task} cross-task prompting brings significant improvement compared to zero-shot prompting. The best overall source-target pair improves the performance by 162\% for Llama2-7b, 30\% for Llama2-13b and 7\% for GPT3.5. Different models give the best performance in different source-target pairings. Not all pairs of source-target coupling seem to work, for example, Commonsense-QA as a source task decreases performance on Financial-phrasebank but is the best source task for ARC-Challenge and MedMCQA (for Llama2-7b). But what could be observed is that token classification tasks (POS and NER) seem to depreciate cross-task prompting for Llama2-13b and GPT3.5, their performance for Llama2-7b is also sub-par compared to other source-target pairings. Race and ARC-Easy seem to be robust source task that improves performance for any target task. ARC-Easy, MNLI and BoolQ can also be considered to have this robustness as they only hurt the performance in one or two cases.

On average, cross-task prompting improves performance by 107\% for Llama2-7b, 18.6\% for Llama2-13b and 3.2\% for GPT3.5. This is a strong argument for doing cross-task prompting when we lack labeled target data, especially for small models whose zero-shot abilities are poor~\citep{wei2022chain}. 

\subsection{Cross task generated pseudo-examples vs Gold label}
To see the efficacy of our proposed method in section \ref{sec:Pseudo Label generation cross-task prompting} we utilise a $D_{pl}$ of just size 8 and have three setups to create the examples for $C$:-

\begin{enumerate}
    \item \textbf{Gold-label: } We use the annotated version of $D_{pl}$ for $C$ creation.
    \item \textbf{Pseudo-label(ZS): } We use zero-shot prompting to label $D_{pl}$ and then use examples from it to generate $C$.
    \item \textbf{Pseudo-label(CT): } We use the cross-task method as proposed in section \ref{sec:Pseudo Label generation cross-task prompting} for $C$ generation.
\end{enumerate}

The results of this experiment are noted in Table \ref{tab:pseudo_label}. For Llama models, as evident pseudo labels generated via cross-prompting are substantially better than zero-shot pseudo labels, they are of higher quality and lead to comparable performance as Gold-label. This observation is valid in all the datasets. These results provide us with a good alternative to utilise cross-task prompting unlabeled data for prompting for Llama models. GPT3.5 on the other hand seems to give similar performance for all the three setups.


\begin{table}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{cccc}
\hline
                                         & Gold-label                  & Pseudo-examples(ZS) & Pseudo-examples(CT) \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{C0C0C0}Llama-2-7b}                                                               \\ \hline
ARC-Challenge                            &       $44.4_{0.37}$          &     $7.2_{4.52}$             &          $44.4_{0.37}$                \\
Financial-Phrasebank                     &       $48.4_{9.56}$          &     $56.5_{2.01}$            &          $56.8_{2.37}$   \\
MedMCQA                                  &       $30.6_{0.84}$          &     $21.0_{14.61}$            &          $30.6_{1.03}$                  \\
SciQ                                     &       $67.7_{0.65}$          &     $3.3_{1.88}$             &          $64.6_{1.51}$            \\ 
Social-i-QA                              &       $46.8_{1.69}$          &     $46.7_{1.57}$            &          $46.4_{1.94}$                \\ \hline
Average                                  &       $47.6_{2.62}$          &     $26.9_{4.91}$               &           $48.5_{1.44}$                \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{C0C0C0}Llama-2-13b}                                                               \\ \hline
ARC-Challenge                            &       $56.8_{0.47}$          &     $59.7_{0.84}$             &          $58.4_{1.79}$                \\
Financial-Phrasebank                     &       $67.9_{5.03}$          &     $67.9_{5.03}$            &          $67.99_{5.03}$   \\
MedMCQA                                  &       $38.2_{1.31}$          &     $2.6_{1.8}$            &          $39.4_{0.37}$                  \\
SciQ                                     &       $84.1_{0.75}$          &     $29.3_{39.5}$             &          $84.1_{0.75}$            \\ 
Social-i-QA                              &       $63.6_{2.78}$          &     $43.6_{27.7}$            &          $61.4_{3.66}$                \\ \hline
Average                                  &       $62.1_{2.06}$           &    $40.62_{14.97}$                    & $62.2_{2.32}$                         \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{C0C0C0}GPT3.5}                                                               \\ \hline
ARC-Challenge                            &       $76.7_{0.89}$          &     $77.4_{1.13}$             &          $77.46_{0.94}$                \\
Financial-Phrasebank                     &       $80.4_{4.35}$          &     $86.2_{2.84}$            &          $83.43_{6.41}$   \\
MedMCQA                                 &       $43.2_{5.65}$          &     $43.4_{3.30}$            &          $47.8_{2.97}$                  \\
SciQ                                     &       $92.8_{1.04}$          &     $91.2_{0.56}$             &          $91.5_{0.25}$            \\ 
Social-i-QA                             &       $77.8_{1.06}$          &     $76.6_{0.65}$            &          $76.6_{0.43}$                \\ \hline
Average                                  &          $74.2_{2.59}$       &     $74.9_{1.69}$                    &   $75.3_{2.2}$                       \\ \hline
\end{tabular}
}
\caption{Accuracy in pseudo label generated prompting. Here ZS stands for zero-shot, and CT stands for cross-task. Pseudo-label(CT) performs comparably to Gold-label examples}
\label{tab:pseudo_label}
\end{table}

\begin{table*}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{cccccccccccc}
\hline
\backslashbox{TAR}{SRC} & In-task  & +ARC-Easy & +AG-news & +BoolQ & +Com-QA & +C-POS & +C-NER & +MNLI & +QQP  & +RACE  & +SST2 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}Llama-2-7b}                                                                                \\ \hline
ARC-Challenge        & 49.8 & \textbf{51.2}     & 41.6    & 45.8  & 49.6           & 43.6          & 40.2          & 41.6 & 45.2 & 50.0  & 42.8 \\
Financial-Phrasebank & 33.3 & 33.3     & 33.3    & 33.3  & 33.5           & 33.3          & 34.5          & 35.7 & 33.3 & 34.5  & \textbf{50.3} \\
MedMCQA              & 32.4 & 33.6     & 29.2    & 30.6  & 32.8           & 31.0         & 30.8          & 28.2 & 30.2 & \textbf{34.2}  & 31.2 \\
SciQ                 & 67.4 & \textbf{73.4}     & 60.4    & 68.6  & 71.6           & 59.0          & 57.4          & 58.6 & 57.9 & 71.2  & 62.4 \\
Social-i-QA          & 43.3 & 49.9     & 46.7    & 44.5  & \textbf{58.3}          & 44.7          & 44.3          & 41.5 & 43.9 & 51.7  & 43.1 \\ \hline
Average              & 45.2 & 48.3     & 42.2    & 44.5  & 48.1           & 42.3          & 41.4          & 41.1 & 42.1 & \textbf{48.3} & 45.9 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}Llama-2-13b}                                                                               \\ \hline
ARC-Challenge        & 61.8 & \textbf{63.0}     & 60.8    & 61.6  & 61.0           & 61.2          & 60.0          & 60.0 & 59.6 & 61.2  & 58.8 \\
Financial-Phrasebank & \textbf{86.0} & 77.0     & 71.2    & 77.6  & 82.4           & 65.1          & 69.4          & 75.2 & 64.8 & 81.8  & 85.6 \\
MedMCQA              & 40.2 & 40.8     & 37.6    & 40.4  & 41.0           & 38.2          & 39.0          & 38.6 & 38.6 & \textbf{41.8}  & 37.2 \\
SciQ                 & 84.8 & \textbf{85.8}     & 83.0    & 83.8  & 85.6           & 81.4          & 81.4          & 80.2 & 79.2 & 84.0  & 79.6 \\
Social-i-QA          & 54.8 & \textbf{62.1}     & 52.09   & 52.3  & 60.9           & 53.3          & 53.7          & 54.1 & 53.5 & 61.6  & 53.9 \\ \hline
Average              & 65.5 & 65.7     & 60.9    & 63.1  & 66.2           & 59.8          & 60.7          & 61.6 & 59.1 & \textbf{66.0}  & 63.0 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}GPT3.5}                                                                               \\ \hline
ARC-Challenge        & 78.6      & 78.2     & 78.2    & 78.8  & \textbf{79.8}           & 77.4          & 78.4          & 78.4 & 78.4 & 77.6  & 79.0 \\
Financial-Phrasebank & 75.4      & 80.2     & 79.4    & 79.6  & 83.8           & 70.4          & 80.2          & 80.2 & 81.0 & \textbf{81.6}  & 77.6 \\
MedMCQA              & \textbf{52.0}      & 51.2     & 48.6    & 51.2  & 47.4           & 48.2          & 49.4          & 49.4 & 48.8 & 49.8  & 49.8 \\
SciQ                 & 92.6      & 91.2     & 91.8    & 92.6  & 92.4           & 91.8          & 92.0          & 92.0 & 91.4 & \textbf{93.0}  & 91.6 \\
Social-i-QA          & 75.6      & 77.0     & 76.2    & 74.4  & 76.6           & 76.2          & \textbf{77.4}          & 77.4 & 75.0 & 77.0  & 75.6 \\ \hline
Average              & 74.8      & 75.6     & 74.8    & 75.3  & \textbf{76.0}           & 72.8          & 74.2          & 75.0 & 74.9 & 75.8 & 74.7 \\ \hline
\end{tabular}
}
\caption{Accuracy for in-task combined with cross-task prompting setup, $C$ is created using one source example and one human-labelled target example. Source tasks are mentioned in columns and Target tasks are in rows. (Commonsense-QA, Conll2003-POS, Conll2003-NER abbreviated to Com-QA, C-POS and C-NER resp.)}
\label{tab:cross-task+ICL}
\end{table*}
\subsection{Correlation between source-target pairs}


\begin{figure*}[]
    \centering
    \includegraphics[width=\linewidth]{images/heatmap.png}
    \caption{Cosine similarities between embeddings of the task instructions for source-target pair, extracted from the last hidden layer of (a) Llama-2-7b (b) Llama-2-13b}
    \label{fig:heatmap}
\end{figure*}

One may assume that a pair of similar source and target tasks would lead to better performance. To test this hypothesis, we compare the semantic similarity of embeddings generated by the task instructions of source-target pairs. Figure \ref{fig:heatmap} shows a heat map of this score. We note that for 80\% of the time the source instruction that is the most semantically similar to the target instruction, also serves as its best suiter i.e. leads to the best performance in Table \ref{tab:cross-task}. 

\subsection{Combining in-task prompting with cross-task prompting}

Combining cross-task prompting with human-annotated target examples does improve performance, as seen in Table \ref{tab:cross-task+ICL}. However, we see that this improvement is immensely dependent on the source-target task pair chosen. Unlike Table \ref{tab:cross-task}, we are unable to find robust source datasets that improve the performance throughout the setup. Nevertheless, in multiple source-target instances, there is noteworthy improvement.

\subsection{Increasing number of examples for cross-task prompting}

\begin{figure}[]
\begin{center}
\includegraphics[width=7.5cm]{images/cross-task.png}
\caption{Variation of accuracy with change in the number of examples sampled from $D_s$ for cross-task prompting on Llama2-7b model}
\label{fig:change_in_k_CTICL}
\end{center}
\end{figure}

\todo{I dont like the color combination of Fig 2. Pls change}
\todo{Fig 3 and 4 can be merged. different line patterns needed.}

Unlike in-task prompting \citet{DBLP:journals/corr/abs-2005-14165}, where increasing the number of examples increases prompting performance, cross-task prompting doesn't seem to improve (Fig \ref{fig:change_in_k_CTICL}) with an increase in source examples. For most target tasks increasing source examples does not affect performance while for some the performance decreases.

\subsection{Increasing number of pseudo-examples for in-task prompting}

\begin{figure}[]
\begin{center}
\includegraphics[width=7.5cm]{images/pseudo-label-2.png}
\caption{Variation of accuracy with change in the number of pseudo-label sampled from $D_{pl}$ on Llama2-7b model}
\label{fig:change_in_k_pseudo_CTICL}
\end{center}
\end{figure}

Increasing prompt samples from pseudo labeled $D_{pl}$ increases performance as also seen in \citet{DBLP:journals/corr/abs-2005-14165}, Refer:- Fig.\ref{fig:change_in_k_pseudo_CTICL}

\subsection{Semantically similar vs randomly example selection}
\label{sec:Semantically similar vs randomly demonstrations prompts}

In a cross-task setup, choosing the examples randomly leads to substantially poorer performance than when we generate $C$ of the model with semantically similar examples Ref Table \ref{tab:rand_vs_sim}. More concerning, in many cases it causes 0\% accuracy because the model gets confused.  

\begin{table}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{cccccc}
\hline
\backslashbox{TAR}{SRC} & AG-news      & BoolQ         & Com-QA & \multicolumn{1}{l}{MNLI} & \multicolumn{1}{l}{QQP} \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{C0C0C0}Random}                                                                        \\ \hline
ARC-Challenge        & $26.6_{3.0}$ & $3.7_{0.7}$   & $0.0_{0.0}$    & $29.5_{3.7}$             & $26.8_{2.9}$            \\
Financial-Phrasebank & $0_{0}$      & $1.4_{1.3}$   & $13.9_{14.75}$ & $0.0_{0.0}$              & $0.0_{0.0}$             \\
MedMCQA              & $26.1_{1.5}$ & $20.8_{1.1}$  & $0.0_{0.0}$    & $25.1_{0.9}$             & $25.0_{0.2}$            \\
SciQ                 & $34.5_{3.2}$ & $10.0_{4.25}$ & $0.0_{0.0}$    & $34.0_{4.1}$             & $28.7_{0.8}$            \\
Social-i-QA          & $36.8_{1.3}$ & $0.6_{0.1}$   & $0.0_{0.0}$    & $24.9_{2.7}$             & $29.27_{3.9}$           \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{C0C0C0}Semantically Similar}                                                            \\ \hline
ARC-Challenge        & 36.6         & 35.0          & 43.6           & 34.2                     & 36.4                    \\
Financial-Phrasebank  & 62.1         & 40.9          & 14.6           & 62.7                     & 44.7                    \\
MedMCQA              & 26.8         & 28.0          & 33.0           & 23.0                     & 26.0                    \\
SciQ                 & 45.4         & 49.0          & 65.6           & 44.8                     & 25.4                    \\
Social-i-QA          & 40.1         & 40.3          & 48.5           & 38.9                     & 39.7       \\ \hline            
\end{tabular}
}
\caption{Accuracy when cross-task examples are picked randomly vs when they are pickled semantically similar. Experiments were done on a Llama2-7b model. For random prompting, we generated the results over three seeds. (Commonsense-QA abbreviated to Com-QA.)}
\label{tab:rand_vs_sim}
\end{table}

\subsection{Mixed cross-task prompting}

So far we have seen that cross-task prompting works for single source-target task pairs. But what if we utilise multiple source tasks to make our $C$? Such a context would be diverse. To experiment with such a setup we prompt on Llama models using three methods:-

\begin{enumerate}
    \item \textbf{Best source cross-task:} We select the best source tasks for every target task using Table \ref{tab:cross-task} and sample four semantically similar examples from that source task to create the $C$ for $x_t \in D_t$.
    \item \textbf{Random mixed cross task:} To see if a diverse set of tasks helps in prompting, we randomly sample four source tasks and create $C$ using semantically most similar examples for each $x_t \in D_t$.
    \item \textbf{Best mixed cross task:} This method is a combination of the first two, we use the top four best source tasks from Table \ref{tab:cross-task} and sample a semantically similar source example from the task to make our $C$.
\end{enumerate}

As evident from Table  \ref{tab:mixed_prompting}, a mixed prompting mechanism does not perform better than single-source task prompting, on the contrary, it seems to hurt the performance of the model, in fact, single-source task prompting with only one example (Table \ref{tab:cross-task}) seems to do better than these mixed prompts method. It seems diversity leads to the model getting more confused thus hurting its performance.

\begin{table}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{cccc}
\hline
                                         & Best source cross-task                  & Random mixed cross task & Best mixed cross task \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{C0C0C0}Llama-2-7b}                                                               \\ \hline
ARC-Challenge                            &        $51.6$                &     $42.8$             &          $44.0$                \\
Financial-Phrasebank                     &        $64.7$          &     $48.3$            &          $56.0$   \\
MedMCQA                                  &         $34$          &     $28.6$            &          $29.0$                  \\
SciQ                                     &        $46.2$          &     $60.5$             &          $67.2$            \\ 
Social-i-QA                              &        $42.7$          &     $42.9$            &          $42.9$                \\ \hline
Average                                  &       $47.84$          &     $44.62$               &           $47.8$                \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{C0C0C0}Llama-2-13b}                                                               \\ \hline
ARC-Challenge                            &        $66.4$                &     $57.2$             &          $60.4$                \\
Financial-Phrasebank                     &        $76.6$          &     $71.4$            &          $61.5$   \\
MedMCQA                                  &         $38.4$          &     $38.3$            &          $41.2$                  \\
SciQ                                     &        $84.6$          &     $80.5$             &          $84.2$            \\ 
Social-i-QA                              &        $49.3$          &     $61.9$            &          $61.27$                \\ \hline
Average                                  &       $47.6_{2.62}$          &     $61.8$               &           $61.7$                \\ \hline
\end{tabular}
}
\caption{Accuracy in mixed cross-task prompting. The number of examples to create $C$ is four in all setups.}
\label{tab:mixed_prompting}
\end{table}



\subsection{Error Section} \label{error-analysis}
We see four types of error occurring in cross-task prompting (refer to Table \ref{tab:error-analysis} for the examples). They are categorised as follows:
\begin{enumerate}
    \item \textbf{Label space replication:} In example \#1, the source example is from the \textit{Conll2003-POS} dataset, a POS tagging task. In contrast, the target task is to predict the financial sentiment analysis. So, the generation should be either negative, positive or neutral but we observe that the output is a sequence of POS tags instead. Here, the LLM is replicating the label space of the source task and the definition of the target task is not able to guide it to the correct target label space.
    
    \item \textbf{Junk prediction:} In some cases we observe that the output is neither from the label space of the source task nor from that of the target task. As in example \#2, the source task is to classify each token into one named entity category (NER), and the target task is to predict the financial sentiment. The output in this case is found to be junk - it is a sequence of \textit{N}'s but \textit{N} is not a pre-defined named entity category, neither is it a label for the target task. Further, we observe that the correct label in this example is 'neutral' - the LLM could not follow the target task instruction provided and gets confused between the correct prediction label of the target task and the token classification task where the output is expected to be a sequence of labels, and instead outputs a sequence with the initial letter of the correct label.
    
    \item \textbf{Copying effect:} We also see the copying effect, which has been observed by \citet{zicl}, where the predicted label is the same as the label of the context example which is semantically very similar to the target input. In example \#3, the target input is semantically very similar to the context example from the source task provided in the prompt, and consequently, the LLM incorrectly outputs the same label as that of the context example.
    
    \item \textbf{Instruction not followed:} We observe that in some instances the LLM does not adhere to the instruction given in the form of task definition for the target task. In example \#4, the LLM is supposed to output one among the four options \textit{A}, \textit{B}, \textit{C}, \textit{D}, instead it outputs the text corresponding to the option \textit{D} - though \textit{D} is the correct answer in this case, the LLM is not able to follow the instruction properly and the output is not in the desired target label space.
\end{enumerate}

\begin{table*}[!t]
\small
\begin{center}
\scalebox{0.9}{
\begin{tabular}{ |m{0.1cm}|m{13cm}| m{2.5cm}|}
 \hline
 \#&{\bf Prompt}&{\bf Output} \\
  \hline
1.&Definition: Given a sentence do token classification by doing Part-of-speech (POS) tagging, ... categories.

Sentence: Net profit 6.08 vs 3.98 

Label: JJ NN CD NNP CD

Definition: Given a sentence ... label the sentence as "negative", "positive" or "neutral"

Sentence: Consolidated net sales increased 16 \% ... to a loss of EUR0 .7 m in the prior year period. 
 
 Label:  & \textcolor{red}{NNP CD NNP CD} \\
\hline
2.&
Definition: Given a sentence do token classification ... till the entity ends.

Sentence: Total shares to be offered 2.5 million 

Label: O O O O O O O

Definition: Given a sentence ... label the sentence as "negative", "positive" or "neutral"

Sentence: The offer of some 30 million shares ... expected to be completed by Oct. 9 , Outokumpu said . 

Label: & \textcolor{red}{N N N N N N N} \\
\hline
3.&Definition: Given a question answering task ... most appropriate choice that answers the question

Question: Which object in our solar system reflects light and is a satellite that orbits around one planet?

A. Earth

...

D. the Moon 

Answer: D

Definition: Given a question answering task ... most appropriate choice that answers the question

Question: Which of the following sets contains only objects that shine as a result of reflected light?

A. moons, planets, and comets

...

D. planets, stars, and moons 

Answer: & \textcolor{red}{D} \\
\hline
4.&Definition: Given a context and a question ... answer in a "True" and "False".

Context: A blacklight (or often black light), also referred to as a UV-A light, ... much visible light. 

Question: is a black light and an ultraviolet light the same thing 

Answer: True

Definition: Given a question from a scientific exam ... provide the label "A", "B", "C" and "D" as answer

Question: When exposed to ultraviolet, ... characteristic visible wavelengths, a process called this?

A. pigment

...

D. fluorescence 

Answer: & \textcolor{red}{fluorescence}\\
\hline
\end{tabular}
}
\caption{Error analysis of cross-task prompting. Four examples represent the major error characteristics (discussed in Section \ref{error-analysis}). The outputs shown are generated by Llama-2-13b. The examples shown here are shortened, complete examples are provided in Table \ref{tab:error-analysis-complete} of Appendix \ref{sec:appendix}.}
\vspace{-2mm}
\label{tab:error-analysis}
\end{center}
\end{table*}


==> semantic_cross-task_old.tex <==
\section{Prompting Techniques}
\label{sec:cross-task-method}

In this section, we outline our approach for cross-task prompting.

{\bf Task definition} for a given task is a natural language instruction for the LM describing what is asked of it (see Figure~\ref{fig:change_in_k_psudo_CTICL} for example). Since a cross-task setup would result in in-context examples from different tasks (with different label spaces), such a definition is necessary to discriminate.

Next, given two datasets \(D_s\) and \(D_t\) corresponding to two different tasks with task definitions \(d_s\) and \(d_t\), respectively, we formalize the cross-task prompting as inferring the output \(\hat{y}_t\) for an input \(x_t\in D_t\) conditioned upon a demonstration from \(D_s\):
\begin{equation*}
\small
    \hat{y}_t = \underset{y}{\mathrm{argmax}}\, p(y|(d_s \oplus x_s \oplus y_s \oplus d_t \oplus x_t))
\end{equation*}
% \subsection{Preliminaries}
In this setup, we denote \(D_s\) and \(D_t\) as source and target task datasets, respectively. Note that the formalization is equivalent to 1-shot prompting where the only provided example input-output pair comes from a different dataset. Table \ref{tab:cross-task-prompts} of Appendix \ref{sec:appendix} presents illustrative examples of prompts in this setup. Our experiments suggest that \(>\)1-shot setup in cross-task prompting does not improve (and often deteriorates) performance. 

\citet{liu-etal-2022-makes} showed that for a target input $x_t$, generating $C$ from semantically similar examples leads to not only better results but also a more robust method of prompting. Similarly, \citet{tanwar-etal-2023-multilingual} showed that ICL could be done in a cross-lingual setup by aligning the semantic and task signals of the source and target languages.

\if 0
Let $D_{t}={(d_t,x_{t}^i)}_i$ be a dataset in a domain-specific task $T_{t}$, where $x_t^i$ is the target input and $d_t$ is the task definition. We want to label this target dataset $D_t$ of task $T_t$ using examples from a labeled source dataset $D_{s}={(d_s,x_{s}^i,y_{s}^i)}_i $, where input examples $x_{s}^i$ taken from the source task  $T_{s}$, $y_t^i$ its corresponding correct answer and $d_s$ its task definition. More concretely, cross-task prompting is a method of solving $T_t$ by leveraging examples from a source task $T_s$, by selecting $k$ examples from $T_s$ to construct the prompt-context $C$:
    $$C= i_{t}\oplus x_{s}^1\oplus y_{s}^1\oplus[sep]\oplus \cdots x_{s}^k\oplus y_{s}^k,$$
where $[sep]$ is a separator token (e.g., newlines), and $\oplus$ denotes the concatenation operator. A prompt $P$ is created conditioned on $C$, $x_t^i$ and $d_t$, to generate label $y_t^i$ corresponding to $x_t^i \in D_t$, i.e., 
$$y_t=\llm(y|C\oplus [sep]\oplus d_t\oplus x_t).
$$
Examples of cross-task prompts can be seen in Table \ref{tab:cross-task-prompts} of Appendix \ref{sec:appendix}.

%\todo{vanilla in-context learning is not a subset of cross-task. \textcolor{red}{Rephrased}}

\textbf{In-context learning} is a popular method of prompting in which $C$ is generated from a labeled $D_{t}$; in our setup, we assume unavailability of labeled $D_{t}$. Similarly, \textbf{zero-shot prompting} prompts the model without any $C$, i.e., passing the model only the target input and assigning the generation as $y_t$. We propose cross-task prompting as an alternative scenario that does better than zero-shot prompting. Both prompting methods have been used as baselines in our work to check the efficacy of cross-task prompting.

\subsection{Semantically similar example selection}
\label{sec: Semantic-based cross-task prompting}
 
\citet{liu-etal-2022-makes} showed that for a target input $x_t$, generating $C$ from semantically similar examples %experimented with semantically similar prompting showing that utilising semantically similar input examples, from a labeled target dataset, to the target examples $x_t$ in creating the $C$ 
leads to not only better results but also a more robust method of prompting. Similarly, \citet{tanwar-etal-2023-multilingual} showed that ICL could be done in a cross-lingual setup by aligning the semantic and task signals of the source and target languages. They empirically showed that choosing semantically similar examples along with manually created task aligners leads to better cross-lingual adaptation of source and target language tasks. 

\begin{algorithm}\small
\SetAlgoLined
\caption{Semantic cross-task prompting}\label{alg:sim-prompt}
\textbf{Input: }Target input $x_t$, source data $D_s$, task definitions $d_t$ and $d_s$, sentence encoder $\theta$, and number of samples to extract $k$.

\textbf{Procedure: }
$\mathbf{e_{t}}\gets\theta(x_t)$\\
\For{$x^s\in D_s$}{
    $\mathbf{e_{s}^i}\gets\theta(x_{s}^i)$
    
    $s_i\gets\frac{\mathbf{e_{t}.e_{s}^i}}{||e^{t}||_2||e_s^{i}||_2}$}
    
Select top $k$ sentences based on $s_i$ 

$C\gets d_s\oplus x_{s}^1\oplus y_{s}^1\oplus[sep]\oplus \cdots x_{s}^k\oplus y_{s}^k$

$y_{t}=\llm(y|C\oplus [sep]\oplus d_t\oplus x_t)$
\end{algorithm}
\fi

Drawing inspiration from these works, we set up the cross-task prompting regime with sampling examples $x_s$ from the source task dataset $D_s$ that are semantically similar to the target input $x_t$.
To extract semantically similar examples, we first utilize Sentence Transformer \cite{reimers-2019-sentence-bert} to extract the sentence embedding of target and source inputs. Following this, based on the cosine similarity between the embeddings, we select top source examples. %\todo{we have context, input, labels. What is exemplar?}
% Algorithm \ref{alg:sim-prompt} shows a concise implementation of the method.



{\bf In-task examples combined with cross-task prompting. }
\label{sec:In-task prompting combined with cross-task prompting}
So far, we have assumed the unavailability of any labeled target dataset. But, if we do have a labeled target example, could prepending a source task boost its prompting performance?

To emulate such a scenario,
%\todo{dont write anotators; otherwise people will be confused. we are not doing any annotation} 
a labeled example from the target dataset is sampled. This 
 labeled example $(x_{lt},y_{lt}),\ \text{where}\ x_{lt} \in T_t$, is then used to construct prompt. This mixed setup can be formalized as,
\begin{equation*}
\small
    \hat{y}_t = \underset{y}{\mathrm{argmax}}\, p(y|(d_s \oplus x_s \oplus y_s \oplus d_t \oplus x_{lt} \oplus y_{lt} \oplus x_t))
\end{equation*}
 
Examples of prompts are provided in Table \ref{tab:icl-with-cross-task} of Appendix \ref{sec:appendix}.

 

\section{Results and Analysis}
\label{sec:results}

\begin{table*}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{lccccccccccc}
\hline
 \backslashbox{TAR}{SRC}& Zero-shot & ARC-Easy & AG-news & BoolQ & Com-QA & C-POS & C-NER & MNLI & QQP  & RACE  & SST2 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 7B}                                                                                \\ \hline
ARC-Challenge        & 4.6       & \textbf{43.6}     & 33.6    & 35.0  & \textbf{43.6}           & 33.8          & 34.2          & 34.2 & 36.4 & 42.8  & 33.2 \\
Financial-Phrasebank & 34.1      & 43.5     & 62.1    & 40.9  & 14.6           & 1.4           & 0.4           & 62.7 & 44.7 & 53.4  & \textbf{65.0} \\
MedMCQA              & 4.2       & 31.4     & 26.8    & 28.0  & \textbf{33.0}           & 26.2          & 24.0          & 23.0 & 26.0 & 31.6  & 23.2 \\
SciQ                 & 8.0       & 59.0     & 45.4    & 49.0  & \textbf{65.6}           & 34.4          & 29.7          & 44.8 & 25.4 & 64.4  & 39.0 \\
Social-i-QA          & 41.1      & 44.3     & 40.1    & 40.3  & 48.5           & 38.9          & 39.1          & 38.9 & 39.7 & \textbf{49.1}  & 39.3 \\ \hline
Average              & 18.4      & 44.3     & 41.6    & 38.6  & 40.71          & 26.9          & 25.5          & 40.7 & 34.4 & \textbf{48.3} & 39.9 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 13B}                                                                               \\ \hline
ARC-Challenge        & 52.0      & \textbf{59.2}     & 50.6    & 54.6  & 57.4           & 50.6          & 49.8          & 49.2 & 52.8 & 56.8  & 50.8 \\
Financial-Phrasebank & 65.4      & 66.6     & 78.6    & 65.8  & 61.7           & 2.2           & 13.17         & 79.0 & \textbf{82.4} & 66.5  & 72.8 \\
MedMCQA              & 9.2       & 37.2     & 34.2    & 36.6  & 38.8           & 31.6          & 32.6          & 30.2 & 30.6 & \textbf{39.0}  & 31.4 \\
SciQ                 & 55.8      & \textbf{83.4}     & 76.2    & 80.2  & \textbf{83.4}           & 76.4          & 78.6          & 77.2 & 71.2 & 82.8  & 72.6 \\
Social-i-QA          & 55.3      & 60.8     & 55.8    & 56.5  & 63.5           & 56.8          & 55.9          & 53.5 & 55.7 & \textbf{63.7}  & 53.1 \\ \hline
Average              & 47.5      & 61.4     & 59.1    & 58.7  & 60.9           & 43.5          & 46.0          & 57.8 & 58.5 & \textbf{61.7} & 56.1 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}GPT3.5}                                                                               \\ \hline
ARC-Challenge        & 74.6      & 77.2     & 74.4    & 77.8  & 76.2           & 70.2          & 70.8          & 75.2 & 74.0 & \textbf{78.2}  & 72.6 \\
Financial-Phrasebank & 57.5      & 79.8     & \textbf{83.6}    & 78.6  & 82.0           & 50.3          & 64.3          & 72.2 & 74.2 & 73.4  & 75.6 \\
MedMCQA              & 49.6      & 49.8     & 48.5    & \textbf{50.0}  & 48.0           & 47.4          & 45.0          & 46.0 & 49.0 & 47.6  & 48.0 \\
SciQ                 & 91.2      & 91.4     & 89.9    & 90.6  & 91           & 87.8          & 82.0          & 88.8 & 89.8 & \textbf{92.2}  & 89.0 \\
Social-i-QA          & 76.0      & 76.2     & 75.8    & 74.0  & 75.2           & 73.2          & 74.0          & 75.8 & 73.0 & \textbf{77.2}  & 74.8 \\ \hline
Average              & 69.8      & \textbf{74.9}     & 74.5    & 74.2  & 74.5           & 65.8          & 67.2          & 71.6 & 72.0 & 73.7 & 72.0 \\ \hline
\end{tabular}
}
\caption{Accuracy for cross-task setup using one source example. Source tasks are mentioned in columns, and target tasks are in rows. Cross-task prompting brings improvement over zero-shot prompting for certain source-target pairs. (Abbreviations: Com-QA \(\rightarrow\) Commonsense-QA, C-POS \(\rightarrow\) Conll2003-POS, C-NER \(\rightarrow\) Conll2003-NER).}
\label{tab:cross-task}
\vspace{-5mm}
\end{table*}

%\todo{Captions for Tables 1 and 2 do not clearly communicate what is show. Please elaborate properly.}
\noindent \textbf{Datasets and experimental setup.}
Our corpus of tasks consists of ten source and five target tasks. We consider ARC-Easy \cite{Clark2018ThinkYH}, AG-news \cite{Zhang2015CharacterlevelCN}, BoolQ \cite{clark-etal-2019-boolq}, Commonsense-QA \cite{talmor-etal-2019-commonsenseqa}, Conll2003-POS \cite{tjong-kim-sang-de-meulder-2003-introduction}, Conll2003-NER \cite{tjong-kim-sang-de-meulder-2003-introduction}, MNLI \cite{N18-1101}, QQP \cite{DBLP:journals/corr/abs-1907-01041}, RACE \cite{lai-etal-2017-race} and SST2 \cite{socher-etal-2013-recursive} to be our source tasks. Our target tasks are ARC-Challenge \cite{Clark2018ThinkYH}, Social-i-QA \cite{DBLP:journals/corr/abs-1904-09728}, SciQ \cite{SciQA2023}, MedMCQA \cite{pmlr-v174-pal22a} and Financial-Phrasebank \cite{Malo2014GoodDO}. In total, this gives us $50$ unique cross-task setups (see Appendix \ref{sec:appendix-dataset} for dataset details. Table \ref{tab:source-task-definitions} and Table \ref{tab:target-task-definitions} of Appendix \ref{sec:appendix} show task definitions corresponding to source and target tasks, respectively). The dataset size is standardised by sampling $10,000$ and $500$ examples for each source and target task, i.e., $|D_s|=10,000$ and $|D_t|=500$. For our experiments, we used the 7-billion and 13-billion variants of LLaMA-2 \cite{touvron2023llama}, and text-davinci-003 \cite{DBLP:journals/corr/abs-2005-14165} referred to as GPT3.5. We set the number of examples used to create cross-task context as one for all our experiments (unless mentioned explicitly). 



\noindent \textbf{Does cross-task prompting work?}
\label{sec:cross-task-main-result}
As evident from Table \ref{tab:cross-task}%\todo{check this, is this table 9?}
, cross-task prompting significantly improves performance compared to zero-shot prompting. The best overall source-target pair improves performance by 162\% for LLaMA-2 7B, 30\% for LLaMA-2 13B and 7\% for GPT3.5. We note that different models give the best performance in different source-target pairs and not all coupling of source-target tasks seem to work; e.g., Commonsense-QA as a source task decreases performance on Financial-Phrasebank, but is the best source task for ARC-Challenge and MedMCQA (for LLaMA-2 7B). Token classification tasks (POS and NER) seem to depreciate performance for LLaMA-2 13B and GPT3.5; their performance for LLaMA-2 7B is also sub-par compared to other source-target pairings. RACE and ARC-Easy are robust source tasks that improve performance for all target tasks in all models. ARC-Easy, MNLI and BoolQ can also be considered to have this robustness to some degree, as they only hurt the performance in one or two cases.

On average, cross-task prompting improves performance by 107\% for LLaMA-2 7B, 18.6\% for LLaMA-2 13B and 3.2\% for GPT3.5. This is a strong argument for prompting in a cross-task manner when we lack labeled target data, especially using small models, which have poor zero-shot abilities ~\citep{wei2022chain}. 

% \todo{All appendix materials should be cited from the main text}

% \todo{same table labels in multiple tables}

\noindent \textbf{Importance of source task definitions.} To further investigate the role of task definitions in cross-task prompting, we check the effect of removing source task definitions on performance. Table  \ref{tab:no_source_inst} reports the average accuracy for all possible source-target pairs corresponding to a task; we note an average drop of 11\% for LLaMA-2 7B and 8\% for LLaMA-2 13B when we prompt without using source task definitions. Hence, definitions play a crucial role in cross-task prompting.

\begin{table}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{lcc}
\hline
                                         & With source definitions                  & W/O source definitions   \\ \hline
\multicolumn{3}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 7B}                                                               \\ \hline
ARC-Challenge                            &        $37.0$                &     $33.0$                           \\
Financial-Phrasebank                     &        $38.8$          &     $27.0$           \\
MedMCQA                                  &         $27.3$          &     $17.06$           \\
SciQ                                     &        $45.7$          &     $48.1$            \\ 
Social-i-QA                              &        $41.8$          &     $42.0$            \\ \hline
Average                                  &       $38.1$          &     $33.8$            \\ \hline
\multicolumn{3}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 13B}                                                               \\ \hline
ARC-Challenge                            &        $53.2$                &     $52.42$              \\
Financial-Phrasebank                     &        $58.9$          &     $48.0$            \\
MedMCQA                                  &         $34.2$          &     $24.36$           \\
SciQ                                     &        $78.2$          &     $75.3$            \\ 
Social-i-QA                              &        $57.5$          &     $58.1$           \\ \hline
Average                                  &       $56.4$          &     $51.6$       \\ \hline
\end{tabular}
}
\caption{Accuracy With and Without(W/O) source definition. We note a drop in accuracy when source definitions are removed.}
\label{tab:no_source_inst}
\vspace{-5mm}
\end{table}

\noindent \textbf{Increasing number of examples for cross-task prompting.}
Unlike in-task prompting \cite{DBLP:journals/corr/abs-2005-14165}, where increasing the number of examples increases prompting performance, in cross-task prompting, performance does not improve with an increase in source examples  (c.f. Fig \ref{fig:k_graph}). For most target tasks, increasing source examples does not affect performance, while for some, the performance decreases.

\noindent \textbf{Semantically similar vs random example selection.}
\label{sec:Semantically similar vs randomly demonstrations prompts}
As shown in Table \ref{tab:rand_vs_sim}, in a cross-task setup, choosing the examples randomly leads to substantially poorer performance than when we generate $C$ of the model with semantically similar examples; concerning is the fact that, in many cases, it causes 0\% accuracy. This may be caused by the model getting confused without any semantic alignment in the prompt.

\begin{table}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{lccccc}
\hline
\backslashbox{TAR}{SRC} & AG-news      & BoolQ         & Com-QA & \multicolumn{1}{l}{MNLI} & \multicolumn{1}{l}{QQP} \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{C0C0C0}Random}                                                                        \\ \hline
ARC-Challenge        & $26.6_{3.0}$ & $3.7_{0.7}$   & $0.0_{0.0}$    & $29.5_{3.7}$             & $26.8_{2.9}$            \\
Financial-Phrasebank & $0_{0}$      & $1.4_{1.3}$   & $13.9_{14.75}$ & $0.0_{0.0}$              & $0.0_{0.0}$             \\
MedMCQA              & $26.1_{1.5}$ & $20.8_{1.1}$  & $0.0_{0.0}$    & $25.1_{0.9}$             & $25.0_{0.2}$            \\
SciQ                 & $34.5_{3.2}$ & $10.0_{4.25}$ & $0.0_{0.0}$    & $34.0_{4.1}$             & $28.7_{0.8}$            \\
Social-i-QA          & $36.8_{1.3}$ & $0.6_{0.1}$   & $0.0_{0.0}$    & $24.9_{2.7}$             & $29.27_{3.9}$           \\ \hline
\multicolumn{6}{c}{\cellcolor[HTML]{C0C0C0}Semantically Similar}                                                            \\ \hline
ARC-Challenge        & 36.6         & 35.0          & 43.6           & 34.2                     & 36.4                    \\
Financial-Phrasebank  & 62.1         & 40.9          & 14.6           & 62.7                     & 44.7                    \\
MedMCQA              & 26.8         & 28.0          & 33.0           & 23.0                     & 26.0                    \\
SciQ                 & 45.4         & 49.0          & 65.6           & 44.8                     & 25.4                    \\
Social-i-QA          & 40.1         & 40.3          & 48.5           & 38.9                     & 39.7       \\ \hline            
\end{tabular}
}
\caption{Accuracy when cross-task examples are picked randomly vs when they are pickled based on semantic similarity. Experiments were done on the LLaMA-2 7B model. For random prompting, we generated the results over three seeds and reported the average performance (Com-QA: Commonsense-QA).}
\label{tab:rand_vs_sim}
\vspace{-5mm}
\end{table}

\begin{table}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{lccc}
\hline
                                         & Best source cross-task                  & Random mixed cross-task & Best mixed cross-task \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 7B}                                                               \\ \hline
ARC-Challenge                            &        $51.6$                &     $42.8$             &          $44.0$                \\
Financial-Phrasebank                     &        $64.7$          &     $48.3$            &          $56.0$   \\
MedMCQA                                  &         $34$          &     $28.6$            &          $29.0$                  \\
SciQ                                     &        $46.2$          &     $60.5$             &          $67.2$            \\ 
Social-i-QA                              &        $42.7$          &     $42.9$            &          $42.9$                \\ \hline
Average                                  &       $47.84$          &     $44.62$               &           $47.82$                \\ \hline
\multicolumn{4}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 13B}                                                               \\ \hline
ARC-Challenge                            &        $66.4$                &     $57.2$             &          $60.4$                \\
Financial-Phrasebank                     &        $76.6$          &     $71.4$            &          $61.5$   \\
MedMCQA                                  &         $38.4$          &     $38.3$            &          $41.2$                  \\
SciQ                                     &        $84.6$          &     $80.5$             &          $84.2$            \\ 
Social-i-QA                              &        $49.3$          &     $61.9$            &          $61.27$                \\ \hline
Average                                  &       $63.06$          &     $61.86$               &           $61.71$                \\ \hline
\end{tabular}
}
\caption{Accuracy in mixed cross-task prompting. The number of examples to create $C$ is four in all setups.}
\label{tab:mixed_prompting}
\vspace{-3mm}
\end{table}

\begin{table*}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{lccccccccccc}
\hline
\backslashbox{TAR}{SRC} & In-task  & +ARC-Easy & +AG-news & +BoolQ & +Com-QA & +C-POS & +C-NER & +MNLI & +QQP  & +RACE  & +SST2 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 7B}                                                                                \\ \hline
ARC-Challenge        & 49.8 & \textbf{51.2}     & 41.6    & 45.8  & 49.6           & 43.6          & 40.2          & 41.6 & 45.2 & 50.0  & 42.8 \\
Financial-Phrasebank & 33.3 & 33.3     & 33.3    & 33.3  & 33.5           & 33.3          & 34.5          & 35.7 & 33.3 & 34.5  & \textbf{50.3} \\
MedMCQA              & 32.4 & 33.6     & 29.2    & 30.6  & 32.8           & 31.0         & 30.8          & 28.2 & 30.2 & \textbf{34.2}  & 31.2 \\
SciQ                 & 67.4 & \textbf{73.4}     & 60.4    & 68.6  & 71.6           & 59.0          & 57.4          & 58.6 & 57.9 & 71.2  & 62.4 \\
Social-i-QA          & 43.3 & 49.9     & 46.7    & 44.5  & \textbf{58.3}          & 44.7          & 44.3          & 41.5 & 43.9 & 51.7  & 43.1 \\ \hline
Average              & 45.2 & 48.3     & 42.2    & 44.5  & 48.1           & 42.3          & 41.4          & 41.1 & 42.1 & \textbf{48.3} & 45.9 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 13B}                                                                               \\ \hline
ARC-Challenge        & 61.8 & \textbf{63.0}     & 60.8    & 61.6  & 61.0           & 61.2          & 60.0          & 60.0 & 59.6 & 61.2  & 58.8 \\
Financial-Phrasebank & \textbf{86.0} & 77.0     & 71.2    & 77.6  & 82.4           & 65.1          & 69.4          & 75.2 & 64.8 & 81.8  & 85.6 \\
MedMCQA              & 40.2 & 40.8     & 37.6    & 40.4  & 41.0           & 38.2          & 39.0          & 38.6 & 38.6 & \textbf{41.8}  & 37.2 \\
SciQ                 & 84.8 & \textbf{85.8}     & 83.0    & 83.8  & 85.6           & 81.4          & 81.4          & 80.2 & 79.2 & 84.0  & 79.6 \\
Social-i-QA          & 54.8 & \textbf{62.1}     & 52.09   & 52.3  & 60.9           & 53.3          & 53.7          & 54.1 & 53.5 & 61.6  & 53.9 \\ \hline
Average              & 65.5 & 65.7     & 60.9    & 63.1  & 66.2           & 59.8          & 60.7          & 61.6 & 59.1 & \textbf{66.0}  & 63.0 \\ \hline
\multicolumn{12}{c}{\cellcolor[HTML]{C0C0C0}GPT3.5}                                                                               \\ \hline
ARC-Challenge        & 78.6      & 78.2     & 78.2    & 78.8  & \textbf{79.8}           & 77.4          & 78.4          & 78.4 & 78.4 & 77.6  & 79.0 \\
Financial-Phrasebank & 75.4      & 80.2     & 79.4    & 79.6  & 83.8           & 70.4          & 80.2          & 80.2 & 81.0 & \textbf{81.6}  & 77.6 \\
MedMCQA              & \textbf{52.0}      & 51.2     & 48.6    & 51.2  & 47.4           & 48.2          & 49.4          & 49.4 & 48.8 & 49.8  & 49.8 \\
SciQ                 & 92.6      & 91.2     & 91.8    & 92.6  & 92.4           & 91.8          & 92.0          & 92.0 & 91.4 & \textbf{93.0}  & 91.6 \\
Social-i-QA          & 75.6      & 77.0     & 76.2    & 74.4  & 76.6           & 76.2          & \textbf{77.4}          & 77.4 & 75.0 & 77.0  & 75.6 \\ \hline
Average              & 74.8      & 75.6     & 74.8    & 75.3  & \textbf{76.0}           & 72.8          & 74.2          & 75.0 & 74.9 & 75.8 & 74.7 \\ \hline
\end{tabular}
}
\caption{Accuracy for in-task combined with cross-task prompting setup; prompt context is created using one source example and one human-labelled target example. Cross-task prompting compliments in-task promoting, leading to better performance (Com-QA: Commonsense-QA, C-POS: Conll2003-POS, C-NER: Conll2003-NER).}
\label{tab:cross-task+ICL}
\vspace{-5mm}
\end{table*}

\noindent \textbf{Mixed cross-task prompting.}
So far, we have seen that cross-task prompting works for single source-target task pairs. Next, we experiment on using multiple source tasks to construct the prompt context. To explore such a setup, we prompt LLaMA models using three methods:

\begin{enumerate}[leftmargin=*,noitemsep,topsep=0pt]
    \item \textbf{Best source cross-task:} We select the best source task for every target task using Table \ref{tab:cross-task} and sample four semantically similar examples from that source task.
    \item \textbf{Random mixed cross task:} To see if a diverse set of tasks helps in prompting, we randomly sample four source tasks and construct the prompt using most semantically similar examples.
    \item \textbf{Best mixed cross task:} This method is a combination of the first two; we use the top four best source tasks from Table \ref{tab:cross-task} and sample semantically similar source examples from each task.
\end{enumerate}

 Table  \ref{tab:mixed_prompting} shows that a mixed prompting mechanism does not perform better than the ``best source cross-task'' prompting method. On the contrary, it seems to hurt the performance of the model; in fact, single-source task prompting with only one example (Table \ref{tab:cross-task}) seems to do better than mixed prompting. Diversity seems to lead the model to get more confused, thus hurting its performance.

\noindent \textbf{Combining in-task with cross-task prompting.} Combining cross-task prompting with labeled target examples improves performance, as seen in Table \ref{tab:cross-task+ICL}; apart from Financial-Phrasebank in LLaMA-2 13B and MedMCQA in GPT3.5 for all other instances there exist a source task that improves the performance when coupled with the in-task example. However, we see that this improvement is immensely dependent on the source-target task pair chosen and unlike Table \ref{tab:cross-task}, we are unable to find robust source datasets that improve the performance throughout the setup. Nevertheless, in multiple source-target instances, there is a noteworthy improvement. In Table~\ref{tab:in-task-comparison}, we compare the outcomes of best mixed task prompting (from Table~\ref{tab:cross-task+ICL}) vs. 1-shot and 2-shot in-task prompting. We can see that, even 2-shot in-task prompting can often deteriorate performance from 1-shot setup while mixed task prompting is able to deliver comparable or better performance. Typically, with relative smaller models like the LLaMA-2 series, betterment with mixed setup is much more profound.
\begin{table}[!t]
\centering
\adjustbox{max width=1\linewidth}{
\begin{tabular}{lcccc}
\hline
Target Task &In-task 1-shot & Cross-task 1-shot &In-task 2-shot & Mixed task 2-shot\\ \hline
\multicolumn{5}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 7B} \\ \hline
ARC-Challenge                                                                             & 49.8 & 43.6   & 53      & 51.2                                            \\
Financial-Phrasebank                                                                      & 33.3   & 65.0                                  & 33.3                                           & 50.3                                            \\
MedMCQA                                                                                   & 32.4    & 33.0                         & 35.2                                           & 34.2                                            \\
SciQ                                                                                      & 67.4    &    65.6                & 75.6                                           & 73.4                                            \\
Social-i-QA                                                                               & 43.3    &    49.1                          & 51.7                                           & 58.3                                            \\

\hline
\multicolumn{5}{c}{\cellcolor[HTML]{C0C0C0}LLaMA-2 13B}\\ \hline
ARC-Challenge                                                                             & 61.8       & 59.2                  & 63                                             & 63                                              \\
Financial-Phrasebank                                                                      & 86        & 82.4                 & 68                                             & 77                                              \\
MedMCQA                                                                                   & 40.2    & 39.0                               & 37.8                                           & 40.8                                            \\
SciQ                                                                                     & 84.8    & 83.4                                & 85.6                                           & 85.8                                            \\
Social-i-QA                                                                               & 54.8   & 63.7                                 & 60.5                                           & 62.1                                            \\

\hline
\multicolumn{5}{c}{\cellcolor[HTML]{C0C0C0}GPT3.5}                                                               \\ \hline
ARC-Challenge                                                                             & 78.6    & 78.2                                 & 78                                             & 79.8                                            \\
Financial-Phrasebank                                                                      & 75.4   & 83.6                                 & 92.4                                           & 81.6                                            \\
MedMCQA                                                                                   & 52    & 50.0                                  & 51.8                                           & 51.2                                            \\
SciQ                                                                                     & 92.6   & 92.2                                  & 94                                             & 93                                              \\
Social-i-QA                                                                               & 75.6   & 77.2                                   & 78.4                                           & 77.4 \\                                          
\hline
\end{tabular}
}
\caption{Accuracy in one-shot in-context learning, two-shot in-context learning and the best performance we achieved when performing cross- and mixed-task prompting (by definition cross-task uses 1-shot example from source task and mixed-task uses a total of 2-shot examples).}
\label{tab:in-task-comparison}
\vspace{-5mm}
\end{table}
